ZeroQ: A Novel Zero Shot Quantization Framework

Quantization is a promising approach for reducing the inference time and memory footprint of neural networks. However, most existing quantization methods require access to the original training dataset for retraining during quantization. This is often not possible for applications with sensitive or proprietary data, e.g., due to privacy and security concerns. Existing zero-shot quantization methods use different heuristics to address this, but they result in poor performance, especially when quantizing to ultra-low precision. Here, we propose ZeroQ , a novel zero-shot quantization framework to address this. ZeroQ enables mixed-precision quantization without any access to the training or validation data. This is achieved by optimizing for a Distilled Dataset, which is engineered to match the statistics of batch normalization across different layers of the network. ZeroQ supports both uniform and mixed-precision quantization. For the latter, we introduce a novel Pareto frontier based method to automatically determine the mixed-precision bit setting for all layers, with no manual search involved. We extensively test our proposed method on a diverse set of models, including ResNet18/50/152, MobileNetV2, ShuffleNet, SqueezeNext, and InceptionV3 on ImageNet, as well as RetinaNet-ResNet50 on the Microsoft COCO dataset. In particular, we show that ZeroQ can achieve 1.71\% higher accuracy on MobileNetV2, as compared to the recently proposed DFQ method. Importantly, ZeroQ has a very low computational overhead, and it can finish the entire quantization process in less than 30s (0.5\% of one epoch training time of ResNet50 on ImageNet). We have open-sourced the ZeroQ framework\footnote{https://github.com/amirgholami/ZeroQ}.

==> _algorithm.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\caption{Pareto frontier optimization}
\label{alg:hutchinson}
    \SetAlgoLined
    \KwInput{ 
    Sensitivity: $\Omega_i(k),~~i\in \{1, 2, \dots, L\}$ \tcp*[]{From~\eref{eq:sensivity_formula}, where $L$ is the total number of layers}\\
    Parameter Size: $P_i,~~i\in \{1, 2, \dots, L\}$ 
    % \tcp*[]{Parameter size for each layer}\\
    $a:$ length of each group \tcp*[]{i.e. each group contains $a$ layers}\\
    $B:$ number of groups \tcp*[]{the total number of groups, i.e. $B=L/a$}\\
    $\tilde{t}:$ candidates used to recompute the sensitivity \tcp*[]{Used to select $t$ candidates based on recomputed sensitivity}\\
    $t:$ number of candidates \tcp*[]{$t < \tilde t$, selected from $\tilde{t}$ configurations based on recomputed sensitivity}\\
    % $\text{Model}=\M, $
    $b:$ number of intervals \tcp*[]{The number of intervals to separate the configuration size}
    }
    
    \KwOutput{
    Best Configuration
    }
    
    
    % results $\leftarrow \varnothing$
    
    \For (\tcp*[]{Finding the ``Best'' configuration in first $i$ blocks}){i = $1,~2,~\dots,~B$}
    {   
        all\_configurations $\leftarrow$ Enumerate($\Omega_{j}$ for $j$ in i-th block)  \tcp*[]{Finding all configurations within $i$-th block exhaustively, $a^{\text{k-bit}}$ in total}
        
        \If {i is $1$}{
            results $\leftarrow$ all\_configurations
            }
        \Else{
            tmp\_results $\leftarrow \varnothing$
            
            \For {config\_prev $\in$ results}{
                \For {config\_curr $\in$ all\_configurations}{
                
                    new\_config $\leftarrow$ \{config\_prev $\cup$ config\_curr\} \tcp*[]{merge config\_prev from first $i-1$ blocks and config\_curr from i-th block to get configurations for first $i$ blocks}
                    % new\_config.$size$  $\leftarrow$ group\_config.$size$ + config.$size$ 
                    
                    % new\_config.$\Omega \leftarrow$ group\_config.$\Omega$ + config.$\Omega$
                    
                    % new\_config.$bit\_setting \leftarrow$ group\_config.$bit\_setting$ $\cup$ config.$bit\_setting$
                    
                    tmp\_results $\leftarrow$ tmp\_results $\cup$ new\_config
                    }
                }
            results $\leftarrow$ tmp\_results
            }
        Divide results into $b$ even interval according to the size of configures from results 

        \tcp*[]{Note that for fast configuration selection, the following two step can be omitted by setting $t=\tilde{t}$}
        
        Recompute top-$\tilde{t}$ configurations in each interval \tcp*[]{Sensitivity recomputation uses the same method as in \eref{eq:sensivity_formula}} 
        
        Select top-$t$ from $\tilde t$ configurations based on recomputed sensitivity
    }
    \Return results
    
    % \For(\ \ \quad \quad\quad\quad\quad\tcp*[]{Hutchinson Steps}){i $=1,2,\ldots$}{
    %     Draw a random vector $v$ from Rademacher distribution (same dimension as $\theta$).
        
    %     Compute $gv = g_\theta^Tv$ \tcp*{Inner product}
    %     Compute $H v$ by backpropagation, $H v = \frac{d(gv)}{d\theta}$ \tcp*{Get Hessian vector product}
    %     Compute and record $v^TH v$
    % }
    % Return the average of all computed $v^TH v$.
\end{algorithm}

==> makefile <==
compilePdfOptions=
compPdftex=pdflatex ${compilePdfOptions}
compile= ${compPdftex}

TARGET=bin/main.pdf
#TARGET= bin/sigconf.pdf
MAIN=main.tex
FILES=main.tex


.SECONDEXPANSION:

####################  COMPILE PDF  ######################

all: ${TARGET}

bin/%.pdf : ${FILES} # .figs_ 
	mkdir -p bin
	#latexmk  -pvc -bibtex -pdf ${MAIN}
	${compile}  $*
	-bibtex $*
	-bibtex $*
	${compile} $*
	${compile} $*
	#${compile} $*
	mv $*.pdf $@
	#make clean
	#open ${TARGET}
	@echo Done ....!


##############  EXTERNALIZE TIKZ-FIGURES  ###############

# TIKZ_FIGS_DIR=tikz_figs
# FIGS=$(shell grep -h '[:space:]*\\inputtikz' ${TIKZ_FIGS_DIR}/figures.tex | sed '1D' | \
#   sed s'/[:space:]*\\inputtikz{\(.*\)}{/\1/' )
# FIGSPDF=$(FIGS:%=%.pdf)
# 
# .figs_ : $(FIGSPDF)
# 	date &> .figs_
# 
# ${TIKZ_FIGS_DIR}/%.pdf : $$(word 1, $$(subst -, ,$${TIKZ_FIGS_DIR}/%)).tex
# 	${compile} --jobname=${TIKZ_FIGS_DIR}/$* \
# 	  '\newcommand{\fakejobname}{${TIKZ_FIGS_DIR}/$*}\input{${TIKZ_FIGS_DIR}/figures.tex}'
# 
########################  CLEAN  ########################

cleanall: clean
	rm -r -f bin/*.pdf ${TIKZ_FIGS_DIR}/*.pdf .figs_
	cd      figs/matlab && ./clean.sh
	cd tikz_figs/matlab && ./clean.sh
	@echo Cleaned All ....! 

clean:
	rm -f *.aux *.dvi *.blg *.bbl *.out *.log */*.log */*/*.log *~ */*~ *.fdb_latexmk *.fls *.xml* *.out
	@echo Cleaned ....! 


